Efficient Parallel Self-Adjusting Computation

Self-adjusting computation is an approach for automatically producing dynamic algorithms from static ones. The approach works by tracking control and data dependencies, and propagating changes through the dependencies when making an update. Extensively studied in the sequential setting, some results on parallel self-adjusting computation exist, but are either only applicable to limited classes of computations, such as map-reduce, or are ad-hoc systems with no theoretical analysis of their performance. In this paper, we present the first system for parallel self-adjusting computation that applies to a wide class of nested parallel algorithms and provides theoretical bounds on the work and span of the resulting dynamic algorithms. As with bounds in the sequential setting, our bounds relate a "distance" measure between computations on different inputs to the cost of propagating an update. However, here we also consider parallelism in the propagation cost. The main innovation in the paper is in using Series-Parallel trees (SP trees) to track sequential and parallel control dependencies to allow propagation of changes to be applied safely in parallel. We show both theoretically and through experiments that our system allows algorithms to produce updated results over large datasets significantly faster than from-scratch execution. We demonstrate our system with several example applications, including algorithms for dynamic sequences and dynamic trees. In all cases studied, we show that parallel self-adjusting computation can provide a significant benefit in both work savings and parallel time.

==> benchmark-descriptions.tex <==
\section{Description of Benchmarks}\label{appendix:benchmarks}

Here, we provide more thorough descriptions of each of our benchmark algorithms.

\paragraph{Spellcheck}

Our first benchmark is a program that computes, for a set of one million strings, the minimum
edit distance of any of those strings to a given reference string. All of the strings in the benchmark
are randomly generated and contain 80 characters. To compute the minimum, we employ a divide-and-conquer-style reduce algorithm.
Our dynamic updates are to modify some set of the strings and recompute the minimum edit distance.
Note that for this benchmark, each modifiable is read only once.

\paragraph{Raytracer}

Our second benchmark is a raytracing algorithm that renders a $2000 \times 2000$ pixel scene consisting of three reflective balls on a flat surface. For each pixel in the image, the algorithm shoots a ray and determines the nearest object that is hit. If that object is reflective, it recursively shoots another ray bouncing off the surface of the object and aggregates the resulting colors, resulting in a reflection. The algorithm performs at most three bounces of reflection. The dynamic update is to modify the color of one ball, which results in its color, and
the color of its reflection in the other balls being updated. In our tested example, this affects a total of
6.25\% of the pixels in the image. One contrasting difference between this and the
edit distance benchmark is that in this case, the input consists of just a constant number of modifiables (the colors of the balls and the walls and floor), but each modifiable
is read by millions of readers. In the edit distance example, there were millions of modifiables but each was read by only a single reader. We therefore do not perform
experiments with varying batch update sizes, since the input size for the problem
is constant. Compared to the edit distance example, we should therefore expect this benchmark to perform more work since it will experience contention on the reader data structure.


\paragraph{String hashing}

Our third benchmark implements a string hashing algorithm commonly employed
by the Rabin-Karp pattern matching method \cite{karp1987efficient}. The algorithm takes
as input a string $S = s_1 s_1 ... s_n$ and computes the value
\begin{equation}
s_1 x^{n-1} + s_2 x^{n-2} + ... + s_n \mod p
\end{equation}
where each character $s_j$ is interpreted as an integer, $x$ is some chosen base,
and $p$ is a large prime. The input string is a randomly generated string of one hundred million characters. Our dynamic updates are to modify a random set of the
characters in the string. This application is similar to our edit distance
example in that it performs divide and conquer on a large string input. What is
different is that in the case of edit distance, the merge steps of the divide-and-conquer
algorithm are extremely cheap to propagate (simply taking the
min of two integers, which will, with $50\%$ probability not even change the value of the result), while in this example, the merge requires more expensive
modular arithmetic computations. For improved granularity, we also split the input
string into chunks of size $64$. This makes the computation much more efficient
since the resulting RSP tree is much smaller, but also has the effect of making change
propagation more expensive since a single update will lead to recomputing the result for $63$ of its unaffected neighbors. Balancing such a tradeoff is a common and very useful technique when implementing self-adjusting algorithms.

\paragraph{Dynamic sequence (List contraction)}

Our next benchmark is an algorithm for
dynamic sequences achieved by dynamizing a static list contraction algorithm. List contraction
has been studied extensively as a parallel pointer-based algorithm and a classic solution to the list ranking problem \cite{karp1990parallel,jaja1992introduction}. List contraction takes as input the elements of a linked list and produces a hierarchical clustering of the elements by deleting randomly chosen
independent sets of elements in successive sequential rounds. By dynamizing this algorithm and allowing the links of the initial
list to be changed, we obtain an algorithm for dynamic sequences that allow us to cut and
rejoin the sequence at arbitrary points, while maintaining some aggregate information over contiguous subsequences. In our example, we maintain the sums of contiguous ranges
of elements. Our input data is a randomized sequence of one million elements, and our dynamic updates are to cut the sequence at randomly chosen locations and
rejoin the pieces together in a randomly chosen order.

Since the algorithm runs for $O(\log(n))$ sequential rounds, we reduce the size
of the RSP tree by processing groups of list elements in small chunks. Specifically,
we group the elements into chunks of size $30$, with which we can use a $32$-bit integer
as a bitset to indicate which elements have not yet been deleted at each round. Not
only does this reduce the size of the RSP tree, and result in improved
granularity, it also allows the algorithm to run much faster in later rounds when most elements have contracted by skipping over empty chunks in constant time. List contraction was studied by Acar et al.~\cite{acar2020batch} in the round-synchronous setting, where it was shown that the computation distance induced by $k$ updates is $O(k\log(1 + n/k))$.


\paragraph{Dynamic trees (Tree contraction)}

Our second-last benchmark is an algorithm for dynamic trees obtained by dynamizing a static
algorithm for tree contraction. Parallel tree contraction was studied by Miller and Reif \cite{miller1985parallel,miller1989parallel,miller1991parallel} in the static context,
as it boasts many applications from parallel expression evaluation to path and subtree
queries on weighted trees. Miller and Reif's tree contraction works by successively applying two operations to the tree: rake, which removes all leaf nodes, and compress, which deletes
a random independent set of vertices that lie on a chain. This results in a cluster 
structure on which data for several useful queries can be augmented. In our implementation,
we maintain the weight of the heaviest edge on the vertex-to-root path for every vertex. We use as input to the algorithm, randomly generated rooted trees with one million vertices of maximum degree $3$ (up to two children per node), since Miller and Reif's algorithm is designed for rooted, bounded-degree trees. Our dynamic updates are to cut a random set of the edges of the tree and replace them with random edges so that the tree remains connected and still satisfies the degree bound.

We use the same trick as in list contraction whereby we process vertices in chunks
of size $30$ to obtain improved granularity, smaller RSP trees, and better performance in later rounds of the algorithm. Finally, we also
note that parallel tree contraction has been studied theoretically in the self-adjusting setting. Recent work by Acar et al.~\cite{acar2020batch} shows that the computation distance between modifying $k$ edges in a forest of size $n$ is $O(k\log(1 + n/k))$, which implies that our automatically dynamized update algorithm performs $O(k\log(n)\log(1+n/k))$ work, only $\log(n)$ slower than the fastest 
parallel batch-dynamic trees algorithms \cite{tseng2018batch,acar2020batch}.

\paragraph{Filter on a BST}

Our final benchmark performs a filter with respect to a given predicate on a binary search tree, returning a new binary search tree consisting only of the elements that satisfy the predicate. In our benchmark, we will the binary search tree with randomly generated integers, and the predicate is to select only the odd numbers.

The binary search tree is implemented using nodes consisting of three modifiables: the value stored at the node, and pointers to the left and right child of the node. For improved practical performance, granularity control is implemented by storing a sequence of values at a leaf node, up to $64$ in our implementation. When a new value is inserted, if it would cause a leaf to exceed its capacity, a new internal node is created and the leaf is split into two leaves.



==> bst.tex <==
\section{Computation Distance of Filter}\label{appendix:computation-distance}

\paragraph{Filter on a Binary Search Tree} 

The self-adjusting BST is implemented as a set of nodes where each node consists of 3 modifiables: one storing the value, and two for storing pointers to the left and right child of the node. All insertions are done at the leaves, and since the insertions are uniformly random, the BST is balanced (has height $O(\log(n))$) w.h.p. \textproc{FILTER} is implemented recursively: given a node we call \textproc{FILTER} on its left and right children, and depending on whether the value satisfies the filter predicate or not, we use the \textproc{JOIN} or \textproc{JOIN2} functions to combine them into one tree. \textproc{JOIN} takes two BSTs $A, B$ and one value $v$ such that for all $a \in A$ we have $a < v$ and for all $b \in B$ we have $v < b$. \textproc{JOIN2} takes two BSTs $A, B$ such that for all $a \in A, b \in B$ we have $a < b$. They both return (via destination passing) one BST with the combined values. \textproc{JOIN} takes $O(1)$ work and \textproc{JOIN2} takes $O(\log(n))$ work w.h.p. Pseudocode for \textproc{FILTER} is given in Algorithm~\ref{alg:filterbst}.
%and pseudocode for the join operations appears in Algorithm~\ref{alg:joinbst}.


\begin{algorithm}
  \caption{Filter on BSTs}
  \label{alg:filterbst}
  \small
  \begin{algorithmic}[1]
    \Function{filter}{t: $\alpha\ \textbf{node*}$, f : $\alpha \mapsto \textbf{bool}$, dest : $\alpha\ \textbf{node } \textbf{mod}$}
    \If{t $=$ \algnull{}}
    \State \algwritemod{dest}{\algnull{}}
    \Else
    \State \alglocal{} fL \algassign{} \algorithmicalloc{}(\textbf{node})
    \State \alglocal{} fR \algassign{} \algorithmicalloc{}(\textbf{node})
    \State \begin{varwidth}[t]{\linewidth}\algorithmicpar{}
    (\function{} $\Rightarrow$ \textbf{with read}(t.left) \algorithmicas{} lc \textproc{filter}(lc, f, fL), \\ \algtab
    \function{} $\Rightarrow$ \textbf{with read}(t.right) \algorithmicas{} rc \textsc{filter}(rc, f, fR))
    \end{varwidth}
    \State \alglocal{} result \algassign{} \textbf{alloc}(\textbf{node})
    \Read{fL, t.val, fR}{l, v, r}
    \If{f(v)}
      \State \textsc{join}(l, v, r, result)
      \State \algwritemod{dest}{result}
    \ElsIf{l $\neq$ \algnull{} \algor{} r $\neq$ \algnull{}}
      \State \textsc{join2}(l, r, result)
      \State \algwritemod{dest}{result}
    \Else\ 
      \algwritemod{dest}{\algnull{}}
    \EndIf
    \EndRead
    
    \EndIf
    \EndFunction
  \end{algorithmic}
\end{algorithm}


\begin{theorem}\label{thm:filter-distance}
Given a BST $A$, consider the computation resulting from the filter operation with respect to a predicate $f$, such that $f$ can be computed in constant time. Then $k$ uniformly random elements can be inserted to $A$ (obtaining $A'$) such that the computation distance between the resulting RSP trees is $O(k \log^2 n)$ w.h.p, where $n$ is the size of the BST after the new elements are inserted.
\end{theorem}


\begin{proofsketch}[Proof sketch of Theorem~\ref{thm:filter-distance}]
  First, note that the parents of newly added nodes that are not themselves newly added nodes will contain a child whose pointer is updated from null to not null. These will affect the reads on Line 7, which previously would trivially return null, and will now instead run \textproc{Filter}s on the new subtrees. In total, these may perform $O(k \log(n))$ work. The results of these \textproc{Filter}s will then subsequently affect the reads on Line 9, which, since they perform a \textproc{join} or \textproc{join2}, may require $O(\log(n))$ work. This update may change the result, dest, or one of its members, which could again affect a subsequent computation. However, such an affected computation must be one that reads an ancestor of $t$, and hence, in the worst case, at most a chain of length $O(\log(n))$ affectations could occur, each of which performs $O(\log(n))$ work to perform a \textproc{join} or \textproc{join2}. In total, the work of all of the re-executed readers is therefore at most $O(k\log^2(n))$.
\end{proofsketch}



==> cpp.tex <==
\myparagraph{Example algorithm} To give a complete example, Figure~\ref{fig:sum-cpp} shows the divide-and-conquer algorithm for parallel sum
that we gave in pseudocode as Algorithm~\ref{alg:parallel_sum}, implemented
in our C++ library. Observe that the translation from pseudocode to our
library is very natural and follows the exact same structure. In particular,
the programmer is not required to know anything about the underlying RSP tree,
and only has to learn the framework's short list of primitives.

\begin{figure}[t]
\begin{mdframed}
\vspace{-.05in}
\begin{lstlisting}
template<typename It>
psac_function(sum, It lo, It hi, Mod<int>* res) {
  if (lo == hi - 1)
    psac_read((auto x), (lo), {
      psac_write(res, x); });
  else {
    auto mid = lo + (hi - lo) / 2;
    auto left = psac_alloc(int);
    auto right = psac_alloc(int);
    psac_par({ psac_call(sum, lo, mid, left); },
             { psac_call(sum, mid, hi, right); });
    psac_read((auto x, auto y), (left, right), {
      psac_write(res, x + y); });
  } }
\end{lstlisting}
\vspace{-.05in}
\end{mdframed}
\caption{An implementation of a parallel sum algorithm}\label{fig:sum-cpp}
\end{figure}

\begin{comment}
\noindent To complete the example, an invocation of this function, along with
the necessary setup required to initialise the modifiables and propagate
a dynamic update might look like this.

\begin{lstlisting}
// Initialise the input
std::array<psac::Mod<int>, 10> A;
for (int i = 0; i < 10; i++) {
  psac_write(&A[i], i);
}
psac::Mod<int> res;

// Run the algorithm -- res contains 55
auto comp = psac_run(sum, A.begin(), A.end(), &res);

// Propagate a dynamic update -- res will now be 57
psac_write(&A[0], 2);
psac_propagate(comp);
\end{lstlisting}
\end{comment}



==> dynamictrees.tex <==
\paragraph{Dynamic Trees.}

Our final benchmark is an algorithm for dynamic trees obtained by dynamizing a static
algorithm for tree contraction. Parallel tree contraction was studied by Miller and Reif \cite{miller1985parallel,miller1989parallel,miller1991parallel} in the static context,
as it boasts many applications from parallel expression evaluation to path and subtree
queries on weighted trees. Miller and Reif's tree contraction works by successively applying two operations to the tree: rake, which removes all leaf nodes, and compress, which deletes
a random independent set of vertices that lie on a chain. This results in a cluster 
structure on which data for several useful queries can be augmented. In our implementation,
we maintain the weight of the heaviest edge on the vertex-to-root path for every vertex. We use as input to the algorithm, randomly generated rooted trees with one million vertices of maximum degree $3$ (up to two children per node), since Miller and Reif's algorithm is designed for rooted, bounded-degree trees. Our dynamic updates are to cut a random set of the edges of the tree and replace them with random edges so that the tree remains connected and still satisfies the degree bound.

We use the same trick as in list contraction whereby we process vertices in chunks
of size $30$ to obtain improved granularity, smaller RSP trees, and better performance in later rounds of the algorithm. Finally, we also
note that parallel tree contraction has been studied theoretically in the self-adjusting setting. Recent work by Acar et al.~\cite{acar2020batch} shows that the computation distance between modifying $k$ edges in a forest of size $n$ is $O(k\log(1 + n/k))$, which
implies that our automatically dynamized update algorithm performs $O(k\log(n)\log(1+n/k))$ work, only $\log(n)$ slower than the fastest 
parallel batch-dynamic trees algorithms \cite{tseng2018batch,acar2020batch}.

The results are depicted in Table~\ref{tab:tree-contraction}. We see that the dynamic updates exhibit strong work savings until the batch sizes reach $10^4$, at which point recomputing from scratch becomes better. The dynamic updates also exhibit strong parallel scaling as the batch sizes increase, resulting in an impressive total speedup.

\begin{comment}
\begin{figure}
  \centering
  \captionsetup{justification=centering}
  
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{plots/tree_contraction-1000000-abs-update-throughput}
    \caption{Dynamic update throughput for the dynamic sequence problem}\label{fig:tree-contraction-throughput}
  \end{subfigure}
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{plots/tree_contraction-1000000-rel-scaling}
    \caption{Speedup of dynamic updates with respect to the static sequential baseline}\label{fig:tree-contraction-speedup}
  \end{subfigure}
  
  \caption{Throughput (in elements per second) and speedup (relative speed increase compared to the sequential baseline) for the dynamic trees benchmarks}\label{fig:tree-contraction}
\end{figure}
\end{comment}


==> editdistance.tex <==
\paragraph{Spellcheck (Minimum edit distance).}

Our first benchmark is a program that computes, for a set of one million strings, the minimum
edit distance of any of those strings to a given reference string. All of the strings in the benchmark
are randomly generated and contain 80 characters. To compute the minimum, we employ a divide-and-conquer-style reduce algorithm.
Our dynamic updates are to modify some set of the strings and recompute the minimum edit distance.
Note that for this benchmark, each modifiable is read only once.

The results of the benchmark are depicted in Table~\ref{tab:edit-distance}.
We observe that the parallel self-adjusting algorithm outperforms the static
sequential algorithm for all update sizes until the size of the entire input.
It also exhibits strong parallel speedup, scaling as the batch sizes
increase up to $10^4$. This results in a good total speedup for all input sizes.

\begin{comment}
\begin{figure}
  \centering
  \captionsetup{justification=centering}
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{plots/edit_distance-1000000-abs-update-throughput}
    \caption{Dynamic update throughput for the edit distance problem}\label{fig:edit-distance-throughput}
  \end{subfigure}
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{plots/edit_distance-1000000-rel-scaling}
    \caption{Speedup of dynamic updates with respect to the static sequential baseline for the edit distance problem}\label{fig:edit-distance-speedup}
  \end{subfigure}
  \caption{Throughput (in strings per second) and speedup (relative speed increase compared to the sequential baseline) for the edit distance benchmark}\label{fig:edit-distance}
\end{figure}
\end{comment}
% 1, 32, and 32ht denote the runtime of the corresponding algorithm on 1 core, 32 cores, and 32 cores with two-way hyperthreading (64 threads) respectively.


==> hashing.tex <==
\paragraph{String hashing.}

Our third benchmark implements a string hashing algorithm commonly employed
by the Rabin-Karp pattern matching method \cite{karp1987efficient}. The algorithm takes
as input a string $S = s_1 s_1 ... s_n$ and computes the value
\begin{equation}
s_1 x^{n-1} + s_2 x^{n-2} + ... + s_n \mod p
\end{equation}
where each character $s_j$ is interpreted as an integer, $x$ is some chosen base,
and $p$ is a large prime. The input string is a randomly generated string of one hundred million characters. Our dynamic updates are to modify a random set of the
characters in the string. This application is similar to our edit distance
example in that it performs divide and conquer on a large string input. What is
different is that in the case of edit distance, the merge steps of the divide-and-conquer
algorithm are extremely cheap to propagate (simply taking the
min of two integers, which will, with $50\%$ probability not even change the value of the result), while in this example, the merge requires more expensive
modular arithmetic computations. For improved granularity, we also split the input
string into chunks of size $64$. This makes the computation much more efficient
since the resulting RSP tree is much smaller, but also has the effect of making change
propagation more expensive since a single update will lead to recomputing the result for $63$ of its unaffected neighbors. Balancing such a tradeoff is a common and very useful technique when implementing self-adjusting algorithms.

The results are shown in Table~\ref{tab:rabin-karp}. We observe that the algorithm exhibits excellent speedup and nearly perfect scaling, with significant work savings for batch sizes up to $10^5$, after which recomputing from scratch becomes superior.

\begin{comment}
\begin{figure}
  \centering
  \captionsetup{justification=centering}

  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{plots/rabin_karp-100000000-abs-update-throughput}
    \caption{Dynamic update throughput for the string hashing problem}\label{fig:rabin-karp-throughput}
  \end{subfigure}
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{plots/rabin_karp-100000000-rel-scaling}
    \caption{Speedup of dynamic updates with respect to the static sequential baseline}\label{fig:rabin-karp-speedup}
  \end{subfigure}
  
  \caption{Throughput (in characters per second) and speedup (relative speed increase compared to the sequential baseline) for the string hashing benchmark}\label{fig:rabin-karp}
\end{figure}
\end{comment}


==> hull.tex <==
\subsection{Convex hulls}




==> listcontraction.tex <==
\paragraph{Dynamic sequences.}

Our second-last benchmark is an algorithm for
dynamic sequences by dynamizing a static list contraction algorithm. List contraction
has been studied extensively as a parallel pointer-based algorithm and a classic solution to the list ranking problem \cite{karp1990parallel,jaja1992introduction}. List contraction takes as input the elements of a linked list and produces a hierarchical clustering of the elements by deleting randomly chosen
independent sets of elements in successive sequential rounds. By dynamizing this algorithm and allowing the links of the initial
list to be changed, we obtain an algorithm for dynamic sequences that allow us to cut and
rejoin the sequence at arbitrary points, while maintaining some aggregate information over contiguous subsequences. In our example, we maintain the sums of contiguous ranges
of elements. Our input data is a randomized sequence of one million elements, and our dynamic updates are to cut the sequence at randomly chosen locations and
rejoin the pieces together in a randomly chosen order.

Since the algorithm runs for $O(\log(n))$ sequential rounds, we reduce the size
of the RSP tree by processing groups of list elements in small chunks. Specifically,
we group the elements into chunks of size $30$, with which we can use a $32$-bit integer
as a bitset to indicate which elements have not yet been deleted at each round. Not
only does this significantly reduce the size of the RSP tree, and result in improved
granularity, it also allows the algorithm to run much faster in later rounds when most elements have contracted by skipping over
empty chunks in constant time.

The results are shown in Table~\ref{tab:list-contraction}. For the dynamic updates, we observe good speedups and the promising work savings. In particular, the self-adjusting algorithm outperforms the static algorithm until the batch sizes reach $10^4$, at which point the parallel speedups also match or exceed those of the static algorithm.

\begin{comment}
\begin{figure}
  \centering
  \captionsetup{justification=centering}

  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{plots/list_contraction-1000000-abs-update-throughput}
    \caption{Dynamic update throughput for the dynamic sequence problem}\label{fig:list-contraction-throughput}
  \end{subfigure}
  \begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=0.9\columnwidth]{plots/list_contraction-1000000-rel-scaling}
    \caption{Speedup of dynamic updates with respect to the static sequential baseline}\label{fig:list-contraction-speedup}
  \end{subfigure}
  
  \caption{Throughput (in elements per second) and speedup (relative speed increase compared to the sequential baseline) for the dynamic sequence benchmark}\label{fig:list-contraction}
\end{figure}
\end{comment}


==> plots.tex <==

\begin{figure*}
\centering
\captionsetup{justification=centering}

  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/edit_distance-1000000-abs-update-throughput}
    \caption{Update throughput for edit distance}\label{fig:edit-distance-throughput}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/rabin_karp-100000000-abs-update-throughput}
    \caption{Update throughput for string hashing}\label{fig:rabin-karp-throughput}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/list_contraction-1000000-abs-update-throughput}
    \caption{Update throughput for dynamic sequences}\label{fig:list-contraction-throughput}
  \end{subfigure}
  
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/tree_contraction-1000000-abs-update-throughput}
    \caption{Update throughput for dynamic trees}\label{fig:tree-contraction-throughput}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[width=\textwidth]{plots/filter-10000000-abs-update-throughput}
      \caption{Update throughput for filter}\label{fig:filter-throughput}
    \end{subfigure}
  
  \caption{Absolute throughput (in input updates per second) vs the batch size of the updates for each benchmark.}\label{fig:all-throughputs}
\end{figure*}

\begin{figure*}
  \centering
  \captionsetup{justification=centering}
  
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/edit_distance-1000000-rel-scaling}
    \caption{Speedup for edit distance}\label{fig:edit-distance-speedup}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/raytrace-1-rel-scaling}
    \caption{Speedup for the raytracer application}\label{fig:raytrace}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/rabin_karp-100000000-rel-scaling}
    \caption{Speedup of string hashing}\label{fig:rabin-karp-speedup}
  \end{subfigure}
  
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/list_contraction-1000000-rel-scaling}
    \caption{Speedup of dynamic sequences}\label{fig:list-contraction-speedup}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/tree_contraction-1000000-rel-scaling}
    \caption{Speedup of dynamic trees}\label{fig:tree-contraction-speedup}
  \end{subfigure}
  \begin{subfigure}{0.33\textwidth}
      \centering
      \includegraphics[width=\textwidth]{plots/filter-10000000-rel-scaling}
      \caption{Speedup of filter}\label{fig:filter-speedup}
    \end{subfigure}
  
  \caption{Relative speedups (compared to the static sequential baseline) vs the number of processors for each benchmark.}

\end{figure*}

==> proofs.tex <==
\section{Proofs}\label{appendix:proofs}

\noindent The following lemmas will be used to prove the correctness of our algorithms
and also serve as a basis for the cost analysis.

\begin{lemma}\label{lem:only_affected}
  Consider an algorithm and its computation on the input $I$, which is subsequently updated to the input $I'$. Running change propagation on the computation re-executes all affected reads in the RSP tree, and re-executes no reader that is not affected.
\end{lemma}

\begin{proof}
  Observe that the change propagation algorithm (Algorithm~\ref{alg:control}) only traverses to a
  node if it has been marked, and that nodes are only marked when at least one of their descendants is a reader who read a value whose value has changed. Consider a read node that is affected. Suppose it was affected because it was written to during the update from $I$ to $I'$. It and its ancestors will therefore be marked before beginning change propagation. Additionally, the node is not subsumed, and hence is not contained in the subtree of an affected reader's computation. Therefore change propagation will reach this node and re-execute it. 
  
  Suppose instead that the reader is affected due to an update to a modifiable that occurred during change propagation. Since modifiables can only be written once, any read of a modifiable
  that is written by a re-executed reader must happen sequentially after the write, otherwise
  there would be a race to read an unwritten modifiable. Therefore, the corresponding
  sequential branch of the RSP tree containing said reader will not have been traversed yet,
  and affecting the reader via a new write will cause it and its ancestors to become marked. Since this node occurs sequentially after the affecting writer and the change propagation algorithm respects sequential dependencies, it will subsequently be visited and re-executed.
  
  Now consider a read node that is not affected. If it is not affected because it read no modifiables that were updated, it will not be marked and hence will not be re-executed. Otherwise, if it is not affected because it is subsumed, it will not be re-executed because the node that subsumed it will be re-executed, which will re-generate a new RSP subtree for its computation, and hence the node will no longer exist. Therefore change propagation re-executes no reader that is not affected.
\end{proof}

\begin{lemma}\label{lem:only_ancestors}
Consider an algorithm and its computation on the input $I$, which is subsequently updated to the input $I'$. Change propagation after updating the input only visits nodes that are affected and their ancestors.
\end{lemma}

\begin{proof}
Recall again that the change propagation algorithm only traverses marked nodes. If a node is marked, it is either a read node that reads a modified value, or the ancestor of one. Suppose that such a node is not an affected read node or the ancestor of one. Then it must be a subsumed read node, or the ancestor of one. Since the corresponding node is subsumed, the change propagation algorithm will destroy the subtree containing it when re-executing the subsuming node, and hence not traverse it. Therefore change propagation only traverses affected read nodes and their ancestors.
\end{proof}

\begin{lemma}\label{lem:rsp_tree_unique_output}
Consider an algorithm and an RSP tree resulting from running the algorithm on some initial input and possibly performing change propagation. The RSP tree uniquely determines the modifiables written to by the algorithm and their values.
\end{lemma}

\begin{proof}
Follows from the fact that computations are deterministic, and the RSP tree records the values read from modifiables. Given a recorded RSP tree, one could simulate the computation by running all read functions while respecting sequential dependencies, and hence determine all outputs to modifiables in the process.
\end{proof}

\paragraph{Proofs of main theorems}

Here, we prove our main correctness and efficiency theorems.

\begin{proof}[Proof of Theorem~\ref{thm:change-prop-correct} (Correctness)]
  We will first show that change propagation results in the correct RSP trees.  
  First, consider the read nodes that are not affected and are not subsumed by an affected read node. Note that such nodes must be cognate and identical in both trees, since if there were any differences, the nodes or one of their ancestors would be marked, and hence they would be either affected or subsumed. By Lemma~\ref{lem:only_affected}, change propagation re-executes all affected reads. Since computations are deterministic, the affected reads produce the same RSP trees when re-executed by change propagation as they would when running the algorithm from scratch.
  
  Since every read node is either affected, subsumed, or neither, in all cases, every read node is cognate and identical in the tree produced by change propagation and the tree produced by running from scratch. The determinism of the computation then implies that the two trees are identical.
  Since change propagation produces the correct RSP tree, the correctness of all written modifiables follows from Lemma~\ref{lem:rsp_tree_unique_output}.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:change-prop-fast} (Efficiency)]
  By Lemmas~\ref{lem:only_affected} and~\ref{lem:only_ancestors}, change propagation re-executes all affected
  readers and traverses only the ancestors of affected readers. The base work required to
  re-execute the readers is $O(W_\Delta)$ by definition. Additionally, the work required
  to traverse and reach the affected readers in the RSP tree is $O(R_\Delta \cdot h)$
  since the number of affected readers is $R_\Delta$. Each operation of the re-executed reader could execute a read which must add itself
  to the reader set of some modifiables. Since our reader sets are implemented using randomized BSTs, each such occurrence costs $O(\log(r))$ w.h.p. This therefore constitutes an additional $O(W_\Delta \cdot \log(r))$ work since each reader reads a constant number of modifiables.
  
  Note that the algorithm may
  also perform work in marking the ancestors of a newly affected read node, but this
  cost can be charged to the work that will be spent on traversing that portion of
  the RSP tree when the change propagation algorithm reaches it. Lastly, each reader
  that is re-executed will need to clean up the subtree of the RSP tree that the
  previous computation created. This takes at most $O(W_\Delta)$ work, plus an
  additional $O(W_\Delta \cdot \log(r))$ work to remove readers from the reader
  sets of modifiables. In total, the work required
  is therefore $O(W_\Delta \cdot \log(r) + R_\Delta \cdot h)$.
  
  We now consider the span of change propagation. Observe that if the span of the
  original computation is $s$, then change propagation can at most perform $s$
  reads and writes to modifiables along the critical path of the computation.
  Each read may require the addition of a reader to the reader set of a mod, which
  costs $O(\log(r))$, and each write could require marking all of the
  ancestors of all of the readers of the modifiable, which takes $O(h + \log(r))$
  span in our model. In cleaning up the subtrees of previous readers, the
  algorithm could also incur the cost of removing readers from the reader sets
  of modifiables, which will lead to at most $O(s \log(r))$ additional span.
  In total, the span of the change propagation algorithm is therefore $O(s (h + \log(r))).$
\end{proof}

==> pseudocode.tex <==




==> raytracing.tex <==
\paragraph{Raytracer.}

Our second benchmark is a raytracing algorithm that renders a $2000 \times 2000$ pixel scene consisting of three reflective balls on a flat surface. For each pixel in the image, the algorithm shoots a ray and determines the nearest object that is hit. If that object is reflective, it recursively shoots another ray bouncing off the surface of the object and aggregates the resulting colors, resulting in a reflection. The algorithm performs at most three bounces of reflection. The dynamic update is to modify the color of the green ball, which results in its color, and
the color of its reflection in the other balls being updated. In our tested example, this affects a total of
6.25\% of the pixels in the image. One contrasting difference between this and the
edit distance benchmark is that in this case, the input consists of just a constant number of modifiables (the colors of the balls and the walls and floor), but each modifiable
is read by millions of readers. In the edit distance example, there were millions of modifiables but each was read by only a single reader. We therefore do not perform
experiments with varying batch update sizes, since the input size for the problem
is constant.

Compared to the edit distance example, this benchmark should perform slightly worse since
it will experience contention on the reader data structure. The results are depicted in
Table~\ref{tab:raytrace}, where we still observe a strong speedup with respect to the number of processors.
Positively, the algorithm does not appear to be bottlenecked by the contention on the reader data structure,
as it continues to scale to $32$ cores and beyond with hyperthreading. The work savings are also very encouraging, as a total of $6.25\%$ of the image needed
to be updated, and the algorithm performed approximately $7\%$ of the work required to recompute from scratch,
which implies that the overhead from self-adjusting computation was well mitigated by the savings.

\begin{comment}
\begin{figure}
  \centering
  \vspace*{1em}
  \includegraphics[width=0.8\columnwidth]{raytracer-scene}
  \caption{The scene rendered by our raytracing benchmark. The dynamic update modifies the color of the green ball, resulting
    in the ball, and its reflections in the other two balls being updated. This affects 6.25\% of the pixels in
    the image.}\label{fig:balls}
\end{figure}


\begin{figure}
  \centering
  \captionsetup{justification=centering}

  \begin{subfigure}{\columnwidth}
    \centering
  \includegraphics[width=0.9\columnwidth]{plots/raytrace-1-rel-scaling}
  \caption{The relative speedup of dynamic updates for the raytracer benchmark}\label{fig:raytrace}
  \end{subfigure}

  \begin{subfigure}{\columnwidth}
    \centering
    \vspace*{1em}
    \includegraphics[width=0.8\columnwidth]{raytracer-scene}
    \caption{The scene rendered by our raytracing benchmark. The dynamic update modifies the color of the green ball, resulting
      in the ball itself, and its reflections in the other two balls being updated. This affects 6.25\% of the total pixels in
      the image.}\label{fig:balls}
  \end{subfigure}
  
  \caption{Speedup (relative speed increase compared to the sequential baseline) for the raytracing benchmark, and the scene that our benchmark renders.}
\end{figure}
\end{comment}


% 1, 32, and 32ht denote the runtime of the corresponding algorithm on 1 core, 32 cores, and 32 cores with two-way hyperthreading (64 threads) respectively.

==> tables.tex <==

\begin{table*}
  \begin{subtable}[t]{\textwidth}
  
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}
    \hline
    \multirow{2}{*}{$n$} & \multirow{2}{*}{$k$} & \multirow{2}{*}{Seq} & \multicolumn{4}{|c|}{Parallel Static} & \multicolumn{4}{|c|}{PSAC Compute} & \multicolumn{6}{|c|}{PSAC Update} \\ \cline{4-17}
    & & & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & WS & T \\ 
    \hline
    \multicolumn{17}{|c|}{\textbf{Edit Distance}}\\
    \hline
    \input{tables/edit-distance.tex}
    %\caption{Benchmark results for the spellcheck (minimum edit distance) benchmark.}\label{tab:edit-distance}
  %\end{subtable}

  %\begin{subtable}[t]{\textwidth}
    \hline
    \multicolumn{17}{|c|}{\textbf{Raytracer}}\\
    \hline
    \input{tables/raytracer.tex}
  %  \caption{Benchmark results for the raytracer benchmark.}\label{tab:raytrace}
  %\end{subtable}

  %\begin{subtable}[t]{\textwidth}
    \hline
    \multicolumn{17}{|c|}{\textbf{Rabin-Karp}}\\
    \hline
    \input{tables/rabin-karp.tex}
  %  \caption{Benchmark results for the string hashing (Rabin-Karp) benchmark. }\label{tab:rabin-karp}
  %\end{subtable}

  %\begin{subtable}[t]{\textwidth}
    \hline
    \multicolumn{17}{|c|}{\textbf{List Contraction}}\\
    \hline
    \input{tables/list-contraction.tex}
  %  \caption{Benchmark results for the dynamic sequence benchmark. }\label{tab:list-contraction}
  %\end{subtable}
  
  %\begin{subtable}[t]{\textwidth}
    \hline
    \multicolumn{17}{|c|}{\textbf{Tree Contraction}}\\
    \hline
    \input{tables/tree-contraction.tex}
  %  \caption{Benchmark results for the dynamic trees benchmark. }\label{tab:tree-contraction}
  %\end{subtable}

  %\begin{subtable}[t]{\textwidth}
      \hline
      \multicolumn{17}{|c|}{\textbf{Filter}}\\
      \hline
      \input{tables/filter.tex}
  %    \caption{Benchmark results for the filter benchmark.}\label{tab:filter}
  
  \end{tabular}
  }
  
  \end{subtable}

  \caption{Numerical benchmark results. SU is the relative speedup of the 32ht benchmark compared to the corresponding 1 core benchmark. WS denotes the \emph{work-savings}, i.e. the relative speedup of the 1 core dynamic benchmark compared to the static sequential benchmark. Total is the total speedup, i.e. the relative speedup of the 32ht benchmark compared to the static sequential algorithm (equivalently, the product of SU and WS).}\label{tab:results}

\end{table*}




==> tables/edit-distance.tex <==
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline
%\multirow{2}{*}{$n$} & \multirow{2}{*}{$k$} & \multirow{2}{*}{Seq} & \multicolumn{4}{|c|}{Parallel Static} & \multicolumn{4}{|c|}{PSAC Compute} & \multicolumn{6}{|c|}{PSAC Update} \\ \cline{4-17} 
% & & & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & WS & T \\ 
$10^6$ & $10^0$ & 36.72s & 36.21s & 1.19s & 908ms & 39.84 &36.89s & 1.20s & 750ms & 49.16 &44us & 45us & 47us & 0.98 & 819.6k & 800.4k \\ 
\hline \ $10^6$ & $10^1$ & - & - & - & - & - &- & - & - & - &445us & 90us & 112us & 4.93 & 82.42k & 406.7k \\ 
\hline \ $10^6$ & $10^2$ & - & - & - & - & - &- & - & - & - &4.36ms & 265us & 208us & 20.92 & 8.41k & 176.0k \\ 
\hline \ $10^6$ & $10^3$ & - & - & - & - & - &- & - & - & - &44ms & 2.03ms & 1.20ms & 36.97 & 827.9 & 30.61k \\ 
%\hline \ $10^6$ & $10^4$ & - & - & - & - & - &- & - & - & - &436ms & 19ms & 11ms & 37.46 & 84.18 & 3.15k \\ 
\hline \ $10^6$ & $10^5$ & - & - & - & - & - &- & - & - & - &4.04s & 167ms & 118ms & 34.08 & 9.10 & 310.2 \\ 
%\hline \ $10^6$ & $10^6$ & - & - & - & - & - &- & - & - & - &37.67s & 1.81s & 1.21s & 31.04 & 0.97 & 30.26 \\ 
%\hline

%\end{tabular}%
%}

==> tables/filter.tex <==
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline 
\multirow{2}{*}{$n$} & \multirow{2}{*}{$k$} & \multirow{2}{*}{Seq} & \multicolumn{4}{|c|}{Parallel Static} & \multicolumn{4}{|c|}{PSAC Compute} & \multicolumn{6}{|c|}{PSAC Update} \\ \cline{4-17} 
 & & & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & WS & T \\ 
\hline \ $10^7$ & $10^0$ & 454ms & 361ms & 17ms & 15ms & 23.00 &628ms & 35ms & 31ms & 19.76 &34us & 105us & 126us & 0.33 & 13.07k & 4.29k \\ 
\hline \ $10^7$ & $10^1$ & - & - & - & - & - &- & - & - & - &271us & 202us & 268us & 1.34 & 1.68k & 2.24k \\ 
\hline \ $10^7$ & $10^2$ & - & - & - & - & - &- & - & - & - &3.54ms & 1.08ms & 1.06ms & 3.33 & 128.3 & 427.3 \\ 
%\hline \ $10^7$ & $10^3$ & - & - & - & - & - &- & - & - & - &24ms & 3.95ms & 4.01ms & 6.12 & 18.83 & 115.2 \\ 
\hline \ $10^7$ & $10^4$ & - & - & - & - & - &- & - & - & - &138ms & 10ms & 8.39ms & 16.52 & 3.28 & 54.18 \\ 
\hline \ $10^7$ & $10^5$ & - & - & - & - & - &- & - & - & - &535ms & 30ms & 23ms & 22.87 & 0.85 & 19.40 \\ 
\hline \ $10^7$ & $10^6$ & - & - & - & - & - &- & - & - & - &994ms & 78ms & 54ms & 18.29 & 0.46 & 8.36 \\ 
%\hline \ $10^7$ & $10^7$ & - & - & - & - & - &- & - & - & - &2.14s & 201ms & 164ms & 12.99 & 0.21 & 2.76 \\ 
%\hline\\
%\end{tabular}%
%}

==> tables/list-contraction.tex <==
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline 
\multirow{2}{*}{$n$} & \multirow{2}{*}{$k$} & \multirow{2}{*}{Seq} & \multicolumn{4}{|c|}{Parallel Static} & \multicolumn{4}{|c|}{PSAC Compute} & \multicolumn{6}{|c|}{PSAC Update} \\ \cline{4-17} 
 & & & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & WS & T \\ 
\hline \ $10^6$ & $10^0$ & 586ms & 647ms & 70ms & 73ms & 8.77 &4.32s & 219ms & 464ms & 19.66 &761us & 629us & 736us & 1.21 & 770.2 & 931.0 \\ 
\hline \ $10^6$ & $10^1$ & - & - & - & - & - &- & - & - & - &5.58ms & 1.65ms & 1.97ms & 3.38 & 105.2 & 355.2 \\ 
\hline \ $10^6$ & $10^2$ & - & - & - & - & - &- & - & - & - &31ms & 3.31ms & 2.95ms & 10.69 & 18.62 & 199.0 \\ 
%\hline \ $10^6$ & $10^3$ & - & - & - & - & - &- & - & - & - &201ms & 14ms & 10ms & 18.53 & 2.91 & 53.94 \\ 
\hline \ $10^6$ & $10^4$ & - & - & - & - & - &- & - & - & - &1.26s & 74ms & 53ms & 23.33 & 0.47 & 10.89 \\ 
\hline \ $10^6$ & $10^5$ & - & - & - & - & - &- & - & - & - &5.11s & 263ms & 195ms & 26.15 & 0.11 & 3.00 \\ 
%\hline \ $10^6$ & $10^6$ & - & - & - & - & - &- & - & - & - &8.45s & 624ms & 492ms & 17.14 & 0.07 & 1.19 \\ 
%\hline
%\end{tabular}%
%}

==> tables/rabin-karp.tex <==
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline 
\multirow{2}{*}{$n$} & \multirow{2}{*}{$k$} & \multirow{2}{*}{Seq} & \multicolumn{4}{|c|}{Parallel Static} & \multicolumn{4}{|c|}{PSAC Compute} & \multicolumn{6}{|c|}{PSAC Update} \\ \cline{4-17} 
 & & & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & WS & T \\ 
\hline \ $10^8$ & $10^0$ & 1.72s & 1.86s & 58ms & 31ms & 58.34 &3.05s & 96ms & 61ms & 49.81 &14us & 16us & 16us & 0.90 & 118.8k & 107.1k \\ 
\hline \ $10^8$ & $10^1$ & - & - & - & - & - &- & - & - & - &134us & 66us & 74us & 2.02 & 12.81k & 25.86k \\ 
%\hline \ $10^8$ & $10^2$ & - & - & - & - & - &- & - & - & - &1.26ms & 162us & 122us & 10.35 & 1.36k & 14.10k \\ 
\hline \ $10^8$ & $10^3$ & - & - & - & - & - &- & - & - & - &12ms & 717us & 512us & 25.17 & 133.3 & 3.36k \\ 
%\hline \ $10^8$ & $10^4$ & - & - & - & - & - &- & - & - & - &103ms & 4.63ms & 3.11ms & 33.16 & 16.68 & 553.0 \\ 
\hline \ $10^8$ & $10^5$ & - & - & - & - & - &- & - & - & - &621ms & 26ms & 18ms & 34.20 & 2.77 & 94.76 \\ 
\hline \ $10^8$ & $10^6$ & - & - & - & - & - &- & - & - & - &2.49s & 108ms & 66ms & 37.27 & 0.69 & 25.73 \\ 
\hline \ $10^8$ & $10^7$ & - & - & - & - & - &- & - & - & - &5.21s & 213ms & 132ms & 39.30 & 0.33 & 12.99 \\ 
%\hline \ $10^8$ & $10^8$ & - & - & - & - & - &- & - & - & - &19.47s & 709ms & 472ms & 41.24 & 0.09 & 3.65 \\ 
%\hline
%\end{tabular}%
%}

==> tables/raytracer.tex <==
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline 
\multirow{2}{*}{$n$} & \multirow{2}{*}{$k$} & \multirow{2}{*}{Seq} & \multicolumn{4}{|c|}{Parallel Static} & \multicolumn{4}{|c|}{PSAC Compute} & \multicolumn{6}{|c|}{PSAC Update} \\ \cline{4-17} 
 & & & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & WS & T \\ 
\hline \ - & - & 2.54s & 2.46s & 80ms & 49ms & 49.32 &13.65s & 520ms & 323ms & 42.24 &112ms & 8.66ms & 7.47ms & 15.08 & 26.44 & 398.8 \\ 
%\end{tabular}%
%}

==> tables/tree-contraction.tex <==
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c |}\hline 
\multirow{2}{*}{$n$} & \multirow{2}{*}{$k$} & \multirow{2}{*}{Seq} & \multicolumn{4}{|c|}{Parallel Static} & \multicolumn{4}{|c|}{PSAC Compute} & \multicolumn{6}{|c|}{PSAC Update} \\ \cline{4-17} 
 & & & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & $1$ & $32$ & $32$ht & SU & WS & T \\ 
\hline \ $10^6$ & $10^0$ & 824ms & 915ms & 85ms & 66ms & 13.85 &4.85s & 242ms & 689ms & 20.02 &698us & 584us & 672us & 1.19 & 1.18k & 1.41k \\ 
\hline \ $10^6$ & $10^1$ & - & - & - & - & - &- & - & - & - &3.28ms & 1.04ms & 1.23ms & 3.14 & 251.7 & 789.4 \\ 
\hline \ $10^6$ & $10^2$ & - & - & - & - & - &- & - & - & - &24ms & 2.29ms & 2.18ms & 11.03 & 34.23 & 377.7 \\ 
%\hline \ $10^6$ & $10^3$ & - & - & - & - & - &- & - & - & - &210ms & 12ms & 10ms & 20.46 & 3.93 & 80.33 \\ 
\hline \ $10^6$ & $10^4$ & - & - & - & - & - &- & - & - & - &1.47s & 79ms & 60ms & 24.33 & 0.56 & 13.68 \\ 
\hline \ $10^6$ & $10^5$ & - & - & - & - & - &- & - & - & - &5.19s & 254ms & 173ms & 29.85 & 0.16 & 4.74 \\ 
%\hline \ $10^6$ & $10^6$ & - & - & - & - & - &- & - & - & - &8.59s & 428ms & 306ms & 28.00 & 0.10 & 2.69 \\ 
%\hline
%\end{tabular}%
%}
